Oort: Efficient Federated Learning via Guided Participant Selection

Federated Learning (FL) is an emerging direction in distributed machine learning (ML) that enables in-situ model training and testing on edge data. Despite having the same end goals as traditional ML, FL executions differ significantly in scale, spanning thousands to millions of participating devices. As a result, data characteristics and device capabilities vary widely across clients. Yet, existing efforts randomly select FL participants, which leads to poor model and system efficiency. In this paper, we propose Oort to improve the performance of federated training and testing with guided participant selection. With an aim to improve time-to-accuracy performance in model training, Oort prioritizes the use of those clients who have both data that offers the greatest utility in improving model accuracy and the capability to run training quickly. To enable FL developers to interpret their results in model testing, Oort enforces their requirements on the distribution of participant data while improving the duration of federated testing by cherry-picking clients. Our evaluation shows that, compared to existing participant selection mechanisms, Oort improves time-to-accuracy performance by 1.2x-14.1x and final model accuracy by 1.3%-9.8%, while efficiently enforcing developer-specified model testing criteria at the scale of millions of clients.

==> sections/appendices_full.tex <==
% !TeX root = ../kuiper-osdi2021.tex
\appendix

% \section{Analysis of Real-world Dataset}
% \label{app:dataset}
% Here we provide a detailed description of the datasets used in the paper. 


% \subsection{Dataset of Samples}

% A summary of statistics for these datasets can be found in Table \ref{table:data-stats}.


% \begin{table}[h]
%     \centering % used for centering table
%     \setlength\arrayrulewidth{1.2pt}
%     \renewcommand{\arraystretch}{1.}
%     \setlength{\tabcolsep}{10pt} % Default value: 6pt
%     \begin{tabularx}{\linewidth}{c c c} 
%     \hline
%     % \hline %inserts double horizontal lines
%     Dataset & \# of Clients & \# of Samples\\ [.8ex] % inserts table
%     %heading
%     \hline % inserts single horizontal line
%     Google Speech \cite{google-speech} & 2,618 & 105,829\\ [.8ex]
%     OpenImage \cite{openimg} & 14,477 & 1,672,231\\ [.8ex]% inserting body of the table
%     %Blog \cite{blog-corpus} & 19,320 & 137,991,726\\ [.8ex]
%     StackOverflow \cite{stack-overflow} & 342,477 &  135,818,730\\ [.8ex]
%     Reddit \cite{reddit} & 1,660,820 &  351,523,459\\ [.8ex]
%     \hline %inserts single line
%     \end{tabularx}
%     \caption{Dataset statistics.} % title of Table
%     \label{table:data-stats} % is used to refer this table in the text
% \end{table}


% \paragraph{Google Speech Commands.} A speech recognition dataset \cite{google-speech} with over ten thousand clips of one-second-long duration. Each clip contains one of the 35 common words (\eg, digits zero to nine, "Yes", "No", "Up", "Down") spoken by thousands of different people. 
% %\todo{How do we preprocess the data to feed model.}

% \paragraph{OpenImage.} OpenImage \cite{openimg} is a vision dataset collected from Flickr, an image and video hosting service. 
% It contains a total of 16M bounding boxes for 600 object classes (\eg, Microwave oven). We clean up the dataset according to the provided indices of clients. In our evaluation, the size of each image is 96 $\times$ 96.

% % \paragraph{Blog.} Blog Authorship Corpus \cite{blog-corpus} is a language modeling dataset built from the collected posts of thousands of bloggers. In our analysis, each blogger is considered as a client.

% \paragraph{Reddit and StackOverflow.} Reddit \cite{reddit} (StackOverflow \cite{stack-overflow}) consists of comments from the Reddit (StackOverflow) website. It has been widely used for language modeling tasks, and we consider each user as a client. 
% In our experiments, we restrict to the 30k most frequently used words, 
% and represent each sentence as a sequence of indices corresponding to these 30k frequently used words. 
% We use Transformers \cite{transformers} to tokenize these sequences with a block size 64.

% In our experiments, we use 90\% of the dataset as the training set, and the rest 10\% as the held-out testing set. 

% \subsection{Dataset of System Performance and Availability}
% \label{app:sys-profile}

% \paragraph{Heterogeneous system performance.}
% We use the AIBench \cite{ai-bench} dataset and MobiPerf \cite{mobiperf} dataset, 
% and visualize these numbers in Fig~\ref{fig:heter-sys}.
% AIBench dataset provides the training time and inference time of different models across a wide range of devices. 
% As specified in real FL deployments \cite{gg-gboard, federated-learning}, 
% we focus on the capability of mobile devices that have > 2GB RAM in this paper. 
% To understand the network capacity of these devices, 
% we clean up the MobiPerf dataset, and analyze the available bandwidth when they are connected with WiFi, which is preferred for FL as well \cite{fl-survey}.
% In our evaluations, we configure the system performance of each client via sampling by the distribution of these profiles.

% \paragraph{Availability of clients.}
% We use a large-scale real-world user behavior dataset \cite{avail-data}. It comes from a popular input method app (IMA) that can be downloaded from Google Play, and covers 136k users and spans one week from January 31st to February 6th in 2020. This dataset includes 180 million trace items (\eg, battery charge or screen lock) and we consider user devices that are in charging to be available, as specified in real FL deployments \cite{federated-learning}.

% \subsection{Simulation Setup}
% \label{app:simulation}
% We employ the traditional deployment of parameter server and workers, which is the mainstream simulation design used in Google \cite{tff} and existing FL researches \cite{semi-sgd, fl-fair, fl-heternet}. The parameter server acts as the central coordinator in FL, and the worker works as the client. Communications between coordinators and clients will travel through the network, though the communication latency is simulated by the profile of available bandwidth. There exists a global virtual clock on the parameter server to mimic different behaviors in FL (\eg, some clients become offline). 

% The statistical performance (\ie, round-to-accuracy) performs in the same way of that in traditional ML, while the duration of each round is simulated with our real-world profiles. After receiving the global model by communicating with the coordinator (\ie, parameter server), the worker will first dump this model to the storage. For the simulation run of each  client, the worker will load the latest model from the storage, and perform training on the dataset of that client. Note that the worker acts as an individual client at a time, and the computation time is also measured in terms of her profile. When the training of each individual client completes, the worker will push updates to the coordinator, including the updated model and virtual clock time spent on this training round. After receiving these updates, the coordinator will pad this clock time to the global clock. Dynamics of system performance are simulated by specifying different computation/communication latency in profile. 


% \section{\name APIs} 
% \label{app:testing-case}

% \begin{figure}[h]
%   \lstinputlisting[xleftmargin=3.5ex,language=Python,label={lst:selector},escapechar=|]{./code/apis.py}
%   \caption{\name APIs for federated training and testing.}
%   \label{code:apis} 
% \end{figure}
% \paragraph{\name APIs.}
% We have implemented \name as a Python library. \name provides simple APIs to abstract away the problem of participant selection, and developers can import \name in their application.
% Figure~\ref{code:apis} summarizes APIs used in training and testing selector. 
% And we explain these APIs with usage examples of both training selector (Figure~\ref{code:training-selector}) and testing selector (Figure~\ref{code:testing-selector}).


% \begin{figure}[h]
%   \lstinputlisting[xleftmargin=3.5ex,language=Python,label={lst:selector},escapechar=|]{./code/testing.py}
%   \caption{Code snippets of FL testing support in \name.}
%   \label{code:testing-selector} 
% \end{figure}

% \paragraph{Usage Examples of Testing Selector.}
% Figure~\ref{code:testing-selector} shows example code snippets for both scenarios.
% With the individual data characteristics, the developer can use the clairvoyant selector by dumping the client information to \name. 
% Note that we use stratified sampling \cite{probablity} to serve queries like ``\emph{50k representative samples}", which  will determine the number of samples in each category, thus paraphrasing such queries in a form of \textit{``[$p_i$, $p_j$] samples of class [i, j]"}. 
% For the non-clairvoyant scenario, \name receives the developer-specified deviation tolerance and the range of number of samples that a client can hold.
% %
% %\paragraph{Enforce fairness across client groups.}

\section{Proving Benefits of Statistical Utility}
\label{app:utility-proof}

We follow the proof of importance sampling to show the advantage of our statistical utility in theory. 
%
%We start by showing the advantage of importance sampling over random sampling. 
The convergence speed of Stochastic Gradient Descent (SGD) can be defined as the reduction $R$ of the divergence of model weight $\bold{w}$ from its optimal $\bold{w^*}$ in two consecutive round $t$ and $t+1$ \cite{importance-sampling, is-icml} :
\begin{align}
R &= \mathbbm{E}\big[\parallel \bold{w_{t}} - \bold{w^*}\parallel_{2}^{2} - \parallel \bold{w_{t+1}} - \bold{w^*}\parallel_{2}^{2} \big]
\label{eq:speed-reduction}
\end{align}
%where $P_{t}$ denotes the sampling distribution of different data bins at time $t$. 

\paragraph{How does oracle sampling help in theory?} 
If the learning rate of SGD is $\eta$ and we use loss function $L$ to measure the training loss between input features $x$ and the label $y$, then $\bold{w_{t+1}}$ = $\bold{w_t} - \eta \nabla L(\bold{w_t}(x_i), y_i)$. We now set the gradient $G_t=\nabla L(\bold{w_t}(x_i), y_i)$ for brevity, then from Eq.~(\ref{eq:speed-reduction}):
%
\begin{align}
R &= -\mathbbm{E}\big[(\bold{w_{t+1}} - \bold{w^*})^{T}(\bold{w_{t+1}} - \bold{w^*}) - (\bold{w_{t}} - \bold{w^*})^{T}(\bold{w_{t}} - \bold{w^*}) \big] \nonumber \\ 
&= -\mathbbm{E}\big[ \bold{w_{t+1}^T}\bold{w_{t+1}} - 2\bold{w_{t+1}}\bold{w^*} - \bold{w_{t}^T}\bold{w_t} + 2\bold{w_{t}}\bold{w^*}\big] \nonumber \\ 
&= -\mathbbm{E}\big[ (\bold{w_t - \eta G_t})^T(\bold{w_t - \eta G_t}) + 2\eta G_t^T\bold{w^*} - \bold{w_t}^T\bold{w_t} \big] \nonumber \\ 
&= -\mathbbm{E}\big[ -2\eta(\bold{w_t}-\bold{w^*})G_t + \eta^2 G_t^T G_t\big] \nonumber \\ 
&= \small{2\eta(\bold{w_t}-\bold{w^*})\mathbbm{E}[G_t] - \eta^2\mathbbm{E}[G_t]^T\mathbbm{E}[G_t] - \eta^2Tr(\mathbbm{V}[G_t]) 
\label{eq:variance-reduction}
}
\end{align}

It has been proved that optimizing the first two terms of Eq.~(\ref{eq:variance-reduction}) is intractable due to their joint dependency on $\mathbbm{E}[G_t]$, however, one can gain a speedup over random sampling by intelligently sampling important data bins to minimize $Tr(\mathbbm{V}[G_t])$ (\ie, reducing the variance of gradients while respecting the same expectation $\mathbbm{E}[G_t]$) \cite{is-nips, importance-sampling}. Here, the oracle is to pick bin $B_i$ with a probability proportional to its importance $|B_i| \sqrt{\frac{1}{|B_i|}\sum_{k \in B_i} \parallel G(k) \parallel^2}$, where $\parallel G(k) \parallel$ is the L2-norm of the unique sample $k$'s gradient $G(k)$ in bin $B_i$ (Please refer to \cite{bin-sampling} for detailed proof). 

\paragraph{How does loss-based approximation help?}
We have shown the advantage of importance sampling by sampling the larger gradient norm data, and next we present a theoretical proof  that motivates our loss-based utility design. 
%
\begin{corollary}
(Theorem 2 in \cite{loss-sampling}). Let $\parallel G(k) \parallel$ denote the gradient norm of any sample $k$, $M=\max{\parallel G(k) \parallel}$. There exists $K>0$ and $C<M$ such that $\frac{1}{K} L(\bold{w}(x_k), y_k) + C \geq \parallel G(k) \parallel$.
% \begin{align}
% \frac{1}{K} L(\bold{w}(x_k), y_k) + C \geq G(k),  \forall k \nonumber
% \end{align}
\end{corollary}

This corollary implies that a bigger loss leads to a large upper bound of the gradient norm. 
To sample data with a larger gradient norm, we prefer to pick the one with bigger loss.
%
Moreover, it has been empirically shown that sampling high loss samples exhibits similar variance reducing properties to sampling according to the gradient norm, resulting in better convergence speed compared to naive random sampling \cite{importance-sampling}.

By taking account of the oracle and the effectiveness of loss-based approximation, we propose our loss-based statistical utility design, whereby we achieve the close-to-optimal statistical performance (\S\ref{eval:eval-breakdown}).

% \section{Privacy Concern in Collecting Feedbacks}
% \label{app:privacy}

% Depending on different requirements on privacy, 
% we elaborate on how \name respects privacy while outperforming existing mechanisms (\S\ref{sec:stats-util}).

% \paragraph{Compute aggregated training loss on clients locally.}
% Our statistical utility of a client relies on the aggregated training loss of all samples on that client. 
% The training loss of each sample measures the prediction uncertainties of model on every possible output (\eg, category), 
% and even the one with a correct prediction can generate non-zero training loss \cite{testing-bias}.
% So it does not reveal raw data inputs. 
% Moreover, it does not leak the categorical distribution either, 
% since samples of the same category can own different training losses due to their heterogeneous input features. 
% Note that even when we consider homogeneous input features, 
% a high total loss can be from several high loss samples, or many moderate loss samples.  


% \begin{figure}[t]
%   \centering
%   {
%     \subfigure[Round to accuracy (MobileNet). \label{fig:noise-rta-m}]{\includegraphics[width=0.49\linewidth]{Figures/eval/noise/mobilenet_noise_rta.pdf}} 
%     \subfigure[Time to accuracy (MobileNet). \label{fig:noise-tta-m}]{\includegraphics[width=0.49\linewidth]{Figures/eval/noise/mobilenet_noise_tta.pdf}}
%     \subfigure[Round to accuracy (ShuffleNet). \label{fig:noise-rta}]{\includegraphics[width=0.49\linewidth]{Figures/eval/noise/shufflenet_noise_rta.pdf}} 
%     \subfigure[Time to accuracy (ShuffleNet). \label{fig:noise-tta}]{\includegraphics[width=0.49\linewidth]{Figures/eval/noise/shufflenet_noise_tta.pdf}}
%   }
%   \caption{\name improves performance even under noise.}
%   \label{fig:noise-kuiper}
% \end{figure}

% \paragraph{Add noise to hide the real aggregated loss.} 
% Even when clients have very stringent privacy concerns on their aggregated loss, 
% clients can add noise to the exact value. 
% Similar to the popular differentially private FL \cite{diff-fl}, 
% clients can disturb their real aggregated loss by adding Gaussian noise (\ie, noise from the Gaussian distribution).
% %
% In fact, \name can tolerate this noisy statistical utility well, 
% owing to its probabilistic selection from the pool of high-utility clients, 
% wherein teasing apart the top-k\% utility clients from the rest is the key. 

% We first prove that \name is still very likely to select high-utility clients even in the presence of noise.
% To pick $K$ participants out of $N$ all feasible clients, there are totally $\tbinom{N}{K}$ possible combinations. 
% We denote these combinations as $X_i$ and sort them $X_1 \leq  \ldots \leq X_n$ by the ascending order of total utility. 
% Adding noise to each client ends up with an accumulated noise on $X_i$. 
% Thereafter, $X_i$ turns to random variables $\bold{X}_i$ that follow the distribution of accumulated noise. 
% Specifically, distribution of $\bold{X}_i$ is equivalent to shifting the distribution of noise horizontally by a constant $X_i$.
% Given that noise added to $X_i$ follows the same distribution, 
% (i) $\bold{X}_i$ experiences the same standard deviation for every $i$;  
% (ii) the expectation of $\bold{X}_i$ is the sum of $X_i$ and the expectation of noise. 
% Note that adding a constant (\ie, the expectation of noise here) to the inequality does not change its properties, 
% so we still have $\mathbbm{E}[\bold{X}_1] \leq  \ldots \leq \mathbbm{E}[\bold{X}_n]$. 
% As such, we are more likely to select high-utility clients (\ie, combination $\bold{X}_i$ with higher $\mathbbm{E}[\bold{X}_i]$) in sampling when picking $i$ with the highest value of $X_i$. 

% We next show the superior empirical performance of \name over its counterparts under noise.
% In this experiment, we add noise from the Gaussian distribution $Gaussian(0, \sigma^2)$, 
% and investigate \name's performance with different $\sigma$. 
% Similar to differential FL \cite{diff-fl}, we define $\sigma=\epsilon \times Mean(real\_value)$, 
% where $Mean(real\_value)$ is the average of real value without noise. 
% Note that we take this $real\_value$ as reference for the ease of presentations, 
% and developers can refer to other values.
% As such, a large $\epsilon$ implies larger variance in noise, 
% thus providing better privacy by disturbing the real value significantly.
% We report the statistical efficiency after adding noise to the statistical utility (Fig~\ref{fig:noise-rta-m} and Fig~\ref{fig:noise-rta}), as well as the time-to-accuracy performance (Fig~\ref{fig:noise-tta-m} and Fig~\ref{fig:noise-tta}). We observe that \name still improves performance across different amount of noise, and is robust even when the noise is large (\eg, $\epsilon=5$ is often considered to be very large noise \cite{diff-dp}).

% \paragraph{Rely on gradient norm of batches.}
% For case where clients are even reluctant to report the noisy loss, 
% we introduce an alternative statistical utility to drive our exploration-exploitation based client selection.
% Our intuition is to use the gradient norm of batches to approximate the gradient norm of individual samples $\nabla f(k)$ in the oracle importance $|B_i| \sqrt{\frac{1}{|B_i|}\sum_{k \in B_i} \parallel \nabla f(k) \parallel^2}$.
% In mini-batch SGD, we have   
% \begin{align}
% \vspace{-.4cm}
% \bold{w}_{t+1} = \bold{w}_{t} - learning\_rate \times \frac{1}{batch\_size} \times \sum\limits_{k \in batch} \nabla f(k)\nonumber
% \vspace{-.4cm}
% \end{align}
% where $w_{t}$ is the model weights at time $t$.
% Now, we can use the gradient norm of batches (\ie, $\parallel \bold{w}_{t+1} - \bold{w}_{t} \parallel^2$) to approximate $\parallel \nabla f(k) \parallel^2$, and they become equivalent when the batch size is 1.
% Note that today's FL is already collecting the model updates (\ie, $\bold{w}_{t+1} - \bold{w}_{t}$), 
% so we are not introducing additional information.
% As such, we consider the client with larger accumulated gradient norm of batches to be more important. 

% \begin{figure}[t]
%   \centering
%   {
%     \subfigure[MobileNet. \label{fig:norm-mobilenet}]{\includegraphics[width=0.49\linewidth]{Figures/eval/end-to-end/nsdi/mobilenet_tta_norm.pdf}} 
%     \subfigure[ShuffleNet. \label{fig:norm-shufflenet}]{\includegraphics[width=0.49\linewidth]{Figures/eval/end-to-end/nsdi/shufflenet_tta_norm.pdf}}
%   }
%   \caption{\name outperforms with different utility definitions.}
%   \label{fig:norm-tta}
% \end{figure}


% We report the empirical performance of this approximation and the loss-based statistical utility using YoGi. 
% As shown in Fig~\ref{fig:norm-tta}, \name achieves superior performance over the random selection, and the loss-based utility is better than its counterparts. 
% This is because the approximation accuracy with the norm of batches decreases when using mini-batch SGD, whereas 
% mini-batch SGD is more popular than the single-sample batch in ML.

\section{Fairness of Participant Selection}
\label{app:fairness}


\renewcommand{\arraystretch}{1.3}
\definecolor{Gray}{gray}{0.9}

\begin{table}[t]
\centering % used for centering table
\small
\setlength{\arrayrulewidth}{0.9pt}
\begin{tabularx}{\linewidth}{c c c c c c c c c c} % centered columns (4 columns)
\hhline{-|-|-|-|-|} %inserts double horizontal lines
\multirow{2}{*}{Strategy} & Average  & Worst 5\%  & Best 5\% & Var. of \\ 
  & (\%) & (\%) & (\%) & Accuracy \\
\hhline{-|-|-|-|-|}
Prox  & 67.0 & 30.0 & 88.5 & 170.7 \\
\hhline{-|-|-|-|-|}
Kuiper + Prox  & 72.1 & 37.6 & 93.5 & 153.1\\
\hhline{-|-|-|-|-|}
YoGi  & 63.6 & 27.8 &  85.7 & 173.0 \\
\hhline{-|-|-|-|-|}
Kuiper + YoGi  & 74.8 & 42.9 & 92.9 & 134.1 \\
\hhline{-|-|-|-|-|}
Centralized & 79.5 & 49.8 & 95.4 & 114.6 \\
\hhline{-|-|-|-|-|}
\end{tabularx}
\caption{\name achieves a more fair accuracy distribution across clients (\eg, smaller variance of model accuracy across clients).} 
\label{table:acc-fair}
\end{table}

\paragraph{\name improves the fairness of model accuracy.}
While the FL developer may have different fairness criteria, 
achieving a more fair accuracy distribution across interested clients for that given model is mostly the paramount \cite{fl-survey}. 
We follow the popular metrics to measure the fairness of model accuracy for different strategies \cite{fl-fair, fl-survey}. As shown in Table~\ref{table:acc-fair}, where we test the ShuffleNet model accuracy across all clients after training completes, compared with the random participant selection, \name improves the fairness of model accuracy by   
boosting the model accuracy for both the worst 5\% clients and the best 5\% clients, 
while achieving a smaller variance of model accuracy across all clients.

\begin{table}[t]
\centering % used for centering table
\small
\setlength{\arrayrulewidth}{0.9pt}
\begin{tabularx}{\linewidth}{c c c c c c c c c c} % centered columns (4 columns)
\hhline{-|-|-|-|} %inserts double horizontal lines
Strategy & TTA (h)  & Final Accuracy (\%)  & Var. (Rounds) \\ 
\hhline{-|-|-|-|}
Random  & 36.3  &  57.3 &  0.39 \\
\hhline{-|-|-|-|}
$f$=0   & 5.8  & 64.2  &  6.52 \\
$f$=0.25 & 6.1  &  62.4 & 5.1 \\
$f$=0.5 &  13.1 & 59.7  &  2.03 \\
$f$=0.75 & 25.4  & 58.6  & 0.65 \\
$f$=1   &  30.1 & 57.2  &  0.31 \\
\hhline{-|-|-|-|}
\end{tabularx}
\caption{\name can enforce diverse fairness criteria, where Random reports the performance of random participant selection and the rest reports \name's performance given different fairness knobs ($f$). The variance of rounds reports how fairness is enforced in terms of the number of participating rounds across clients, so a smaller variance implies better fairness. We measure the time to accuracy (TTA) using 57.2\% as the target accuracy.} 
\label{table:round-fair}
\end{table}

\paragraph{\name can enforce developer-preferred fairness.} 
Moreover, we show that \name can flexibly respect other developer preferences on diverse fairness. 
In this experiment, we expect all clients should have participated training with the same number of rounds (Table~\ref{table:round-fair}), implying a fair resource usage \cite{fl-survey}. We train ShuffleNet model on OpenImage dataset with YoGi. 
To this end, we sweep different knobs $f$ to accommodate the developer demands for the time-to-accuracy efficiency and fairness. Namely, we replace the current utility definition of client $i$ with $(1-f)\times Util(i) + f \times fairness(i)$, where $fairness(i)= max\_resource\_usage - {resource\_usage(i)}$. 
Understandably, time-to-accuracy efficiency will significantly decrease as $f\to 1$, 
since we gradually end up with round-robin participant selection, which totally ignores the data utility of clients. 
Note that \name still achieves better time-to-accuracy even when $f\to 1$ as it prioritizes high system utility clients 
in such a round-robin scenario. 
Moreover, we note that \name can enforce these fairness criteria while improving efficiency. 

\section{Determining Size of Participants}
\label{app:group-size}

We next introduce Lemma~\ref{lemma:group-size}, which captures how the empirical value of $\bar{X}$ (\ie, average number of samples of participants for category $X$) deviates from the expectation $E[\bar{X}]$ (\ie, average number of samples of all clients) as the size of participants $n$ varies. 

% We start with the key result for a single category.
%
\begin{lemma}
\label{lemma:group-size}
For a given tolerance on deviation $\epsilon$ and confidence interval $\delta$ for category $X$, the number of participants $n$ we need to achieve $Pr[|\bar{X}-{E}[\bar{X}]| < \epsilon] > \delta$ requires: 
\begin{align}
n \geq (N+1) \times \frac{1}{1-\frac{2N}{\log (1-\delta)} \times (\frac{\epsilon}{\max\{X\}-\min\{X\}})^2}
\label{equ:lower-bound}
\end{align}
where $N$ is the total number of feasible clients, and $\max\{X\}$ and $\min\{X\}$ denote the global maximum and minimum possible number of samples that all clients can hold, respectively.
%The first term $M$ depicts the expectation, while the rest capture the skewness of distributions and confidence.
\end{lemma}
Lemma~\ref{lemma:group-size} is a corollary of Hoeffding-Serfling Bound \cite{concentration}, and we omit the detailed proof for brevity. 
Intuitively, when we have an extremely stringent requirement (\ie, $\epsilon \to 0$), we have to include more participants (\ie, $n\to N$).
When more information of the client data characteristics is available, one can refine this range better. For example, the bound of Eq. (\ref{equ:lower-bound}) can be improved with Chernoff’s inequality \cite{concentration} when the distribution of sample quantities is provided.

Similarly, the multi-category scenario proves to be an instance of multi-variate Hoeffding Bound.
Given the developer-specific requirement on each category, 
the developer may want to figure out how many participants needed to satisfy all these requirements simultaneously 
(\eg, $Pr[|\bar{X}-{E}[\bar{X}] | < \epsilon{_x} \wedge |\bar{Y}-{E}[\bar{Y}] | < \epsilon{_y}] > \delta$).  
More discussions are out of the scope of this paper, but readers can refer to \cite{mutivariate-hoeff} for detailed discussions and a complete solution.


% \section{MILP Formula for Testing Selector}
% \label{app:testing-milp}
% For each category $i(\in I)$ of interest, the developer has preference $p_i$ (preference constraint), and an upper limit $B$ (referred to as budget) on how many participants she can have \cite{inspect-fl}.\footnote{$B \rightarrow \inf$ represents a hypothetical case where FL can run on all clients.} 
% %
% Each participant $n(\in {N})$ can contribute $n_i$ samples out of her capacity $c{_n}{^i}$ (capacity constraint). 
% Given her compute speed $s_n$, the available bandwidth $b_n$ and the size of data transfers $d_n$, 
% we aim to minimize the duration of model testing:
% %
% \vspace{-.2cm}
% \begin{align}
% &\min\Big{\{\max\limits_{n \in N}\Big({\frac{\sum_{i \in I}{n_i}}{s_n} + \frac{d_n}{b_n}}\Big)}\Big\} \tag*{$\triangleright$ Minimize duration} \\[-.6\jot] 
% \textrm{s.t.} \quad &\forall i \in I, \sum_{n \in N} n_i = p_i \tag*{$\triangleright$ Preference Constraint}\\[-.7\jot] 
% &\forall i \in I, \forall n \in N, n_i \leq c_n^i \tag*{$\triangleright$ Capacity Constraint}\\[-.4\jot] 
% &\forall i \in I, \sum_{n \in N} \mathbbm{1}(n_i > 0) \leq B \tag*{$\triangleright$ Budget Constraint} 
% \label{eq:lp-testing}
% \end{align} 
% %
% \vspace{-.4cm}

% The max-min formulation stems from the fact that testing completes after aggregating results from the last participant. 
% To enforce fairness (\ie, each client group should contribute a certain number of samples) while optimizing the duration of model testing in our clairvoyant selector, 
% \name can still apply our greedy heuristic in \S\ref{sec:clairvoyant} to select participants by treating each given quota of samples (\eg, the product of the total number of samples and fair share of each group) for each group as an individual query.

% \section{Model Testing on Large-Scale Datasets}
% \label{app:large-testing}

% \begin{figure}[h]
%   \centering
%   {
%     \subfigure[StackOverflow (0.3M clients).]{\includegraphics[width=0.49\linewidth]{Figures/eval/lp/soloverheadso.pdf}} 
%     \subfigure[Reddit (1.6M clients).]{\includegraphics[width=0.49\linewidth]{Figures/eval/lp/soloverheadreddit.pdf}}
%   }
%   \caption{\name scales to millions of clients, while MILP did not complete any query.}
%   \label{fig:test-macro}
% \end{figure}

% Using the same setting used on OpenImage dataset (\S\ref{eval:testing-clair}), we investigate \name's performance on the large-scale StackOverflow and Reddit dataset with millions of clients, 
% where we take 1\% of the global data as the requirement, 
% and sweep the number of interested categories from 1 to 5k. 
% Figure~\ref{fig:test-macro} shows even though we gradually magnify the search space of participant selection by introducing more categories, 
% \name can serve our requirement in a few minutes at the scale of millions of clients, while MILP fails to generate the solution decision for any query. 


%\paragraph{\name improves time-to-accuracy performance while enforcing fairness.}

% \section{More Sensitivity Experiments}
% \label{app:sen-analysis}


% \begin{figure}[t]
%   \centering
%   {
%     \subfigure[ShuffleNet (Image). \label{fig:1k-shuffleround}]{\includegraphics[width=0.49\linewidth]{Figures/eval/end-to-end/nsdi/1k_shufflenet_rta.pdf}} \hfill
%     \subfigure[Albert (LM). \label{fig:1k-lmround}]{\includegraphics[width=0.49\linewidth]{Figures/eval/end-to-end/lm1kround.pdf}}
%   }
%   \caption{More participants may not imply better efficiency.}
%   \label{fig:1k-round-accuracy}
% \end{figure}

% \paragraph{Impact of number of participants $K$.}
% Figure~\ref{fig:1k-round-accuracy} shows the statistical rounds-to-accuracy performance with different size of participants. We notice diminishing rewards in round-to-accuracy performance when taking $K$ = 1000.
% Although admitting more participants in each round can learn a better approximation of the hypothetical updates contributed by all participants, 
% this approximation error decreases sharply as more participants get involved \cite{batchsize-iclr}. 
% This again highlights the importance of participant selection, wherein \name still outperforms the baseline.

% \section{Performance of Non-Clairvoyant Selector}
% \label{app:nc-eval}

% We present a detailed analysis of the performance of non-clairvoyant selector in (\S\ref{eval:non-clair}).

% \begin{figure}[t]
%   \centering
%   {
%     \subfigure[OpenImage. \label{fig:nc-openimg}]{\includegraphics[width=0.49\linewidth]{Figures/eval/non-clair/openimg/dev.pdf}} 
%     \subfigure[\todo{StackOverflow.} \label{fig:nc-so}]{\includegraphics[width=0.49\linewidth]{Figures/eval/non-clair/so/dev.pdf}}
%   }
%   \caption{\name caps data deviation by picking a client subset. Shadow in each figure indicates the max-min range of the y-axis values over 1000 runs given the same x-axis input.}
%   \label{fig:testing-nc-dev}
% \end{figure}

% As shown in Figure~\ref{fig:testing-nc-dev}, for every given deviation target (\ie, y-axis value), \name determines the number of participants needed (\ie, x-axis value). 
% Given the same number of clients, we repeat the random selection over 1000 times to get the real deviation, and care about whether \name can satisfy the requirement on each category.  
% To this end, we report the maximum deviation across all categories of each run in the y-axis. 
% For each given target deviation, we take the maximum number of clients needed in real sampling as the optimal. 
% Due to lack of information, we observe \name will always overcommit selected clients. 
% However, given the size generated by \name, the deviation is always capped in real. 
% \ie, Kuiper will always satisfy the developer requirements on data. 
% Note that when the individual data characteristics are available, our clairvoyant selector can satisfy the exact requirement with little deviation.

%But we note that one straw-man solution is to, 
%Note that different categories are independent to each other most of the time. 

